SAC-MoE: Reinforcement Learning with Mixture-of-Experts for Control of Hybrid Dynamical Systems with Uncertainty

Hybrid dynamical systems result from the interaction of continuous-variable dynamics with discrete events and encompass various systems such as legged robots, vehicles and aircrafts. Challenges arise when the system's modes are characterized by unobservable (latent) parameters and the events that cause system dynamics to switch between different modes are also unobservable. Model-based control approaches typically do not account for such uncertainty in the hybrid dynamics, while standard model-free RL methods fail to account for abrupt mode switches, leading to poor generalization. To overcome this, we propose SAC-MoE which models the actor of the Soft Actor-Critic (SAC) framework as a Mixture-of-Experts (MoE) with a learned router that adaptively selects among learned experts. To further improve robustness, we develop a curriculum-based training algorithm to prioritize data collection in challenging settings, allowing better generalization to unseen modes and switching locations. Simulation studies in hybrid autonomous racing and legged locomotion tasks show that SAC-MoE outperforms baselines (up to 6x) in zero-shot generalization to unseen environments. Our curriculum strategy consistently improves performance across all evaluated policies. Qualitative analysis shows that the interpretable MoE router activates different experts for distinct latent modes.

==> fainekos-macros2.tex <==
% Some macros for temporal logic robustness papers.
% G. Fainekos - Last update 2009.10.09

\RequirePackage{amsfonts}
\RequirePackage{amsmath}

\let\proof\relax 
\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{xpatch}

\makeatletter
\def\thm@space@setup{\thm@preskip=0pt
	\thm@postskip=0pt}
\makeatother


%



\makeatletter
\def\thm@space@setup{%
	\thm@preskip=10pt
	\thm@postskip=0pt%\thm@preskip % or whatever, if you don't want them to be equal
}
\makeatother

\makeatletter
\xpatchcmd{\proof}{\topsep6\p@\@plus6\p@\relax}{}{}{}
\makeatother

\RequirePackage{thmtools}

%\declaretheorem{theorem} 
%\declaretheoremstyle[%
%spaceabove=-6pt,%
%spacebelow=6pt,%
%headfont=\normalfont\itshape,%
%postheadspace=1em,%
%qed=\qedsymbol%
%]{mystyle} 
%\declaretheorem[name={Proof},style=mystyle,unnumbered,
%]{prf}

% \RequirePackage{amsthm}
\RequirePackage{amstext}
\RequirePackage{amssymb}
\RequirePackage{latexsym}

%% Graphics
\RequirePackage{graphicx}
\RequirePackage{todonotes}

%\usepackage{color,soul}
\usepackage{etoolbox}
\newbool{HIGHLIGHTCHANGES}
\newcommand \yhl[1]{\ifbool{HIGHLIGHTCHANGES}{\textcolor{blue}{#1}}{#1}}
\newbool{HIGHLIGHTREDCHANGES}
\newcommand \rhl[1]{\ifbool{HIGHLIGHTREDCHANGES}{\textcolor{red}{#1}}{#1}}

\def\Wn{\, \Wc} % the unless temp operator
\def\mmodels{\mathrel|\joinrel\equiv}
\def\dle{[\![} \def\dri{]\!]} % double-brace
\def\dla{\langle \!\langle} \def\dra{\rangle\!\rangle} % double-angles
\def\Un{\, \Uc} % the until temp operator
\def\rUn{\, \overline{\Uc}} % the restricted until temp operator
\def\rRl{\overline{\Rc}} % the restricted release temp operator

%Distances
\newcommand \GDF {\mathbf{d_h}}
\newcommand \GDFzero {\mathbf{d_h^0}}
\newcommand \dhinf {d_h^{\infty}}
\newcommand \NeighTo[1] {\mathcal{N_{#1}}}
\newcommand \NeighFrom[1] {\mathcal{B_{#1}}}
\newcommand \dist[1] {\mathbf{dist}_{#1}}
\newcommand \prof[1] {\mathbf{depth}_{#1}}
\newcommand \Dist[1] {\mathbf{Dist}_{#1}}
\newcommand{\unsafe}{\mathcal{U}}
\newcommand{\hunsafe}{H_\unsafe}


% System
\newcommand \Sys {\mathcal{H}}
\newcommand \SysFun {\Delta}
\newcommand \SubSysFun {\mathbf{D}}
\newcommand \TDom {\Te}
\newcommand \inpSpace {\mathbf{U}} 
\newcommand \inpSet {U}
\newcommand \inpPt {u}
\newcommand \met {g}
\newcommand \stSet {X}
\newcommand \stPt {x}
\newcommand \sstraj {\mathbf{\stPt}}
\newcommand{\SigSpace}{\stSet^{\TDom}}
\newcommand \ztraj {\mathbf{z}}
\newcommand \hsPt {\eta}
\newcommand \hstraj {\mathbf{\eta}}
\newcommand \hsSet {H}
\newcommand \outSet {Y} 
\newcommand \outPt {y}
\newcommand \outtraj {\mathbf{\outPt}}
\newcommand \hoPt {\phi}
\newcommand \hotraj {\mathbf{\phi}}
\newcommand \graphH {\mathcal{G}}
\newcommand \mode {\ell}
\newcommand \modeSet {L}
\newcommand \guard {G}
\newcommand{\reset}{R}
%General
\newcommand{\such}{\;|\;}
\newcommand \powerset {\mathcal{P}}
\newcommand{\gph}{\text{gph}}




\newcommand \behavior {\mathcal{B}}
\def\dle{[\![} \def\dri{]\!]} % double-brace
\newcommand \abstractor {\sqcup}
\newcommand \abstractand {\sqcap}
\newcommand \bigabstractor {\bigsqcup}
\newcommand \tupleof[1] { \left\langle #1 \right \rangle}
\newcommand \formula \varphi

\newcommand{\Omap}{\Pc(\outSet)^{AP}}
\newcommand{\argmin}{\text{argmin}}
\newcommand{\argmax}{\text{argmax}}

\def\exmpspc{\phi} % symbol for specification used as examples globally in a paper
\newcommand{\unspt}{u}
\newcommand{\Ce}{\mathbb{C}}
\newcommand{\Be}{\mathbb{B}}
\newcommand{\Fe}{\mathbb{F}}
\newcommand{\Me}{\mathbb{M}}
\newcommand{\Ne}{\mathbb{N}}
\newcommand{\Oe}{\mathbb{O}}
\newcommand{\Pe}{\mathbb{P}}
\newcommand{\Qe}{\mathbb{Q}}
\renewcommand{\Re}{\mathbb{R}}
\newcommand{\Se}{\mathbb{S}}
\newcommand{\Te}{\mathbb{T}}
\newcommand{\Ze}{\mathbb{Z}}
\newcommand{\Ve}{\mathbb{V}}
\newcommand{\Xe}{\mathbb{X}}

\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Yc}{\mathcal{Y}}

\newcommand{\Br}{\mathfrak{B}}
\newcommand{\Fr}{\mathfrak{F}}
\newcommand{\Gr}{\mathfrak{G}}
\newcommand{\Ir}{\mathfrak{I}}
\newcommand{\Kr}{\mathfrak{K}}
\newcommand{\Lr}{\mathfrak{L}}
\newcommand{\Rr}{\mathfrak{R}}
\newcommand{\Sr}{\mathfrak{S}}
\newcommand{\Tr}{\mathfrak{T}}
\newcommand{\Ur}{\mathfrak{U}}
\newcommand{\Xr}{\mathfrak{X}}

\newcommand{\Tt}{\mathbb{T}}

% \def\CoRe{\overline{\Re}}
\def\CoRe{\Re\cup\{\pm \infty\}}
\newcommand \staliro {\sc S-TaLiRo}

\newcommand{\BSig}{\Bc(R,X)}
\newcommand{\dsig}{\sigma}
\newcommand{\DSig}{\Fr(N,X)}
\newcommand{\sam}{{\hat \tau}}
\newcommand{\Sam}{\Fr^\uparrow(N,R)}
\newcommand{\SamC}{\Fr^\uparrow_c(N,R)}
\newcommand{\tfun}{\tau}
\newcommand{\TFun}{\Fr^\uparrow(N,\Re_{\geq 0})}
\newcommand{\tss}[1]{\mathbf{#1}}
\newcommand{\TSS}{\DSig \times \TFun}

\newcommand{\st}{\;|\;}
\newcommand{\dom}{\mbox{dom}}
\newcommand{\nnf}{\mathbf{nnf}}
\newcommand{\str}{\mathbf{str}_{\Delta\sam}}
% \newcommand{\trs}{\mathbf{mtc}}
\newcommand{\dur}{\mathbf{dur}}
\newcommand{\mtl}{MTL}
\newcommand{\mitl}{MITL}
\newcommand{\ltl}{LTL}

\newcommand{\FTS}{\Tc}
\newcommand{\SYS}{\Sigma}
\newcommand{\DSYS}{\SYS}
\newcommand{\DASYS}{\mathcal{D}} % Symbol for discrete abstraction
\newcommand{\exmpDASYS}{\DASYS} % symbol for system used as example globally in a paper
\newcommand{\LPV}{\SYS^{\bf LPV}}
\newcommand{\clLPV}{\overline{\SYS}^{\bf LPV}}
\newcommand{\LTI}{\SYS^{\bf LTI}}
\newcommand{\clLTI}{\overline{\SYS}^{\bf LTI}}
\newcommand{\LTV}{\SYS^{\bf LTV}}
\newcommand{\clLTV}{\overline{\SYS}^{\bf LTV}}
\newcommand{\clDSYS}{\overline{\SYS}}
\newcommand{\OmapSYS}{\Fr(AP,\Pc(Y))}

\newcommand{\xinX}{\hat x}
\newcommand{\pinP}{\hat p}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% danger sign
\font\manual=manfnt
\def\dbend{{\manual\char127}} % dangerous bend sign
% Danger, Will Robinson!
\def\danger{\begin{trivlist}\item[]\noindent%
\begingroup\hangindent=3pc\hangafter=-2%\clubpenalty=10000%
\def\par{\endgraf\endgroup}%
\hbox to0pt{\hskip-\hangindent\dbend\hfill}\ignorespaces}
\def\enddanger{\par\end{trivlist}}
% Danger! Danger!
\def\ddanger{\begin{trivlist}\item[]\noindent%
\begingroup\hangindent=3pc\hangafter=-2%\clubpenalty=10000%
\def\par{\endgraf\endgroup}%
\hbox to0pt{\hskip-\hangindent\dbend\kern2pt\dbend\hfill}\ignorespaces}
\def\endddanger{\par\end{trivlist}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\makeatletter
%\def\thm@space@setup{\thm@preskip=5pt
%	\thm@postskip=5pt}
%\makeatother
%\newtheoremstyle{newstyle}      
%{} %Aboveskip 
%{} %Below skip
%{\mdseries} %Body font e.g.\mdseries,\bfseries,\scshape,\itshape
%{} %Indent
%{\bfseries} %Head font e.g.\bfseries,\scshape,\itshape
%{.} %Punctuation afer theorem header
%{ } %Space after theorem header
%{} %Heading
%\theoremstyle{newstyle}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}{Lemma}[section]
%\newtheorem{prop}{Proposition}[section]
\newtheorem{rem}{Remark}[section]
%\newtheorem{prob}{Problem}
%\newtheorem{clm}{Claim}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{challenge}{Challenge}[section]

%\newtheorem{exmp}{Example}

% Ending examples mark
% \newcommand{\exmend}{\hfill \ensuremath{\Box}}
\newcommand{\exmend}{\hfill \ensuremath{\bigtriangleup }}

% Notation for different states of automata
\newcommand{\spaut}{w} % state of a product automaton

\newcommand{\proj}{\mbox{pr}}
\newcommand{\loc}{\mbox{loc}}
\newcommand{\always}{\square}
\newcommand{\eventually}{\Diamond}
\newcommand{\until}{\Uc}
\newcommand{\release}{\Rc}
\newcommand{\defeq}{:=}
